Enhancing Joint Human-AI Inference in Robot Missions: A Confidence-Based Approach

Joint human-AI inference holds immense potential to improve outcomes in human-supervised robot missions. Current day missions are generally in the AI-assisted setting, where the human operator makes the final inference based on the AI recommendation. However, due to failures in human judgement on when to accept or reject the AI recommendation, complementarity is rarely achieved. We investigate joint human-AI inference where the inference made with higher confidence is selected. Through a user study with N=100 participants on a representative simulated robot teleoperation task, specifically studying the inference of robots' control delays we show that: a) Joint inference accuracy is higher and its extent is regulated by the confidence calibration of the AI agent, and b) Humans change their inferences based on AI recommendations and the extent and direction of this change is also regulated by the confidence calibration of the AI agent. Interestingly, our results show that pairing poorly-calibrated AI-DSS with humans hurts performance instead of helping the team, reiterating the need for AI-based decision support systems with good metacognitive sensitivity. To the best of our knowledge, our study presents the first application of a maximum-confidence-based heuristic for joint human-AI inference within a simulated robot teleoperation task.

==> main-sections/background.tex <==
\section{Related Work}
% \an{reference 1,2,4 detail discussion}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/joint-decision-via-metacog.png}
%     \caption{\textbf{Joint Decision-Making Frameworks for Human and Human/AI Dyads}: Each sub-diagram illustrates how individual confidence levels relate to metacognition and decision-making systems. In dyads, a human will exchange confidence levels with their human or AI teammate to make a joint decision.}
%     \label{fig:joint-decision-via-metacog}
% \end{figure}

% \subsection{Metacognitive Sensitivity Sharing}
% Metacognitive sensitivity is also known as metacognitive accuracy or the confidence-accuracy correlation \cite{fleming2014measure}. 


Research on confidence-sharing joint decision-making of dyads began with studies involving two-alternative forced-choice tasks in visual perception within human-human psychology domain. 
% In the psychology domain, systems capable of self-assessing their cognitive processes are referred to as metacognitive systems, which manage confidence levels in their own decision-making processes~\cite{fleming2014measure}. 
Bahrami et al., found that human dyads, by sharing metacognitive sensitivity through confidence levels, achieve significantly better collective output compared to separate individuals~\cite{bahrami2012together}. This phenomenon is termed as two heads better than one. Studies in joint decision-making on varied static tasks such as threat detection~\cite{2hbt1_threatdetection}, detecting fake news~\cite{2hbt1_fakenewsdetection}, deciding rank ordering between items on a survival situation task~\cite{2hbt1_nasasurvival}, and breast and skin cancer diagnosis~\cite{2hbt1_cancerdiagnosis} have also observed similar significant. Recent works \cite{bang2017confidence, rouault2018human} have further explored that the Maximum Confidence Slating (MCS) was used to select the higher confidence choice made in a dyad and it was shown that the joint decision via MCS algorithm resulted in higher accuracy than the best performing individual in the dyads. 

In robotics domain, Raunak et al., demonstrated that confidence plays a crucial role in human-human joint decision-making~\cite{bhattacharyya2024towards}. Further studies by Nguyen et al., demonstrated that the benefit of having two heads remains in robot teleoperation~\cite{nguyen2025group}, even in the absence of communication between participants in a dyad. In this works, the joint decision was determined by human individuals and the decisions guided by the most confident operator via MCS significantly improved joint decision accuracy beyond the best individual's performance. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/robotics-task.png}
    \caption{\textbf{Experiment Setup:} Online robot navigation simulator. Red and green curves show trajectories driven by a participant controlling the Jackal robot under low and high delay conditions, respectively.}
    \label{fig:robot-driving-task}
\end{figure}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/user-interface.png}
    \caption{\textbf{Study Interface:} After completing the robots teleoperation, participants make decision via three panels sequentially: the \textcolor{orange}{left panel} for initial robot choice and confidence, the \textcolor{blue}{middle panel} shows the AI's choices and confidence. If the participant decides to change their initial choice, a third panel, similar to the left, will be shown to collect their final choice and confidence.}
    % This final choice is considered the human's self meta-decision.}
    % \an{human final decision is considered as one kind of meta-decision.}}
    \label{fig:user-interface}
\end{figure*}

In the domain of human-robot interaction, extensive research explores how humans interact with robot to achieve mutual goals and completing given tasks~\cite{chiou2021mixed,hawes2017strands,kunze2018artificial,rigter2020framework}.
Nonetheless, most studies have concentrated on the interaction with the absent of intelligent support systems such as AI-DSS. Unlike static prediction tasks, where decisions rely on fixed data points, dynamic tasks require instantaneous decision-making and adjustments based on fluctuating space and time conditions. Consequently, the domain of mix-initiative where both human-AI play active role in dynamic, spatiotemporal tasks, ubiquitous in human-robot interaction, has yet to be thoroughly explored.

To address this gap in knowledge, our work investigates the impact of AI intelligent decision support systems in the spatiotemporal human-robotics interaction. Motivated by the use of confidence heuristics from human psychology domain, this study is, to the best of our knowledge, the first to examine confidence sharing human-AI systems as well as applying the Maximum Confidence Slating (MCS) algorithm within the human-AI joint decision-making context in the robotics application domain.
% Such a dyadic system is depicted in Fig.\ref{fig:joint-decision-via-metacog}.
% \an{hri $\rightarrow$ meta-decision literature}
Building on the body of related work described above, we identify a gap in the research regarding dyadic joint decision-making in teleoperated robotic tasks, and
% \textbf{Research Questions:} 




% \an{steering the background into hour hri papers. this paper extend hri into 2 dimension: introduced ai element. and 2. focus meta-decision. summarise HRI}

% In their experiments, participants judged which of two briefly-presented stimuli contained an oddball target. 
% They first made their decision individually, then shared their decisions, and if they disagreed, they discussed the matter until they reached a joint decision. 
% The results led to the conclusion that “for two observers of nearly equal visual sensitivity, two heads were definitely better than one provided they were given the opportunity to communicate” 
% In discussing the mechanism for the two-heads-better-than-one (2HBT1) effect, the authors assumed that each individual can monitor the accuracy of their performance and can communicate their confidence accurately to the other member.




==> main-sections/introduction.tex <==
\section{Introduction}


% Joint Decision-Making Frameworks: The diagram shows how confidence levels relate to metacognition and decision-making, with humans and AI exchanging confidence level to make joint decisions.
% The drive for human-AI agent decision-making arises from the complementary strengths and abilities of humans and computing machines.

As we rapidly advance towards an AI-centric future, these AI Decision Support Systems (AI-DSS) are increasingly being utilized in collaboration with humans across a wide spectrum of decision-making domains, including healthcare, business, and design. Since most of these decision aids are deployed in static and passive tasks such as recidivism risk prediction~\cite{dss_whentoadvice}, content moderation~\cite{keswani2021towards}, medical diagnosis~\cite{multiplehumans_ijcai22}, and rental price bidding~\cite{wang2023effects}, little is known about their integration into dynamic, complex domain like robotics. These operational settings often involve high-stakes situations, particularly in teleoperated robotics used for search and rescue operations, medical surgery, military and defense tasks, nuclear and hazardous material handling, and space exploration and maintenance. In this scenarios, decision-making processes are pivotal for achieving optimal control, navigation, and task execution and can have profound impacts on human lives. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/short-meta-2hbt1.png}
    \caption{Joint Decision-Making Framework \raunak{needs more description. Further, is something shared at both levels or only confidence?}}
    % The diagram shows how confidence levels relate to metacognition and decision-making systems, with humans and AI exchanging confidence levels to make joint decisions. The top-level meta-decision determines whose decision becomes the final team choice. \an{remove metacognition system, monitor and control}}
    \label{fig:joint-decision-via-metacog-1}
\end{figure}

% As semi- or fully autonomous teleoperated robots become increasingly integrated into various industries - such as manufacturing (e.g., humanoid robots), healthcare (e.g., surgical robots), transportation (e.g., delivery robots), space exploration, and military applications - the need for precise and reliable real-time decision-making in selecting capable robots for critical missions is crucial. Poor decisions can lead to inefficiencies, safety risks, or even failures in overall robotic operations. Given these high stakes, understanding how humans and AI can best collaborate in selecting capable mission-critical robots is essential and remain challenging, particularly in ensuring that these joint decision-making systems work effectively to improve outcomes in real-time robotic operations. In addition to that, optimizing this partnership to improve overall decision accuracy and efficiency in scenarios involving robot control with different competence levels remains an open problem. 
% \vspace{-10pt}
Early robotic systems involving teleoperation relied solely on human operators as the decision-makers.
Human decision-making, however, often relies on intuition, which can be susceptible to biases, emotions, and incomplete information \cite{casper2003human,norton2017analysis}. 
% \an{check if in HRI-ok no overlap} 
This can result in the gradual degradation of decision-making performance, particularly in complex, fast-paced, and long-term teleoperation scenarios. AI, while powerful, often lacks the contextual understanding and intuition that humans have. Recent advancements have sought to address these limitations by integrating AI with the aim of enhancing decision accuracy through human-AI collaborative decision-making processes, particularly in scenarios involving high cognitive demands~\cite{hawes2017strands,kunze2018artificial,rigter2020framework}. At the outset, human-AI joint decision-making has been managed by a setup with human-initiative control~\cite{chiou2021mixed}, where the final decision to accept or reject the AI recommendation lies with the human operator. Few have delved into the domain of joint decision-making, where both human and AI have an active role, especially in the context of real-time robotics control. 
% \an{we explore meta-decision making by a human or an agent for the mix-initiative human-AI systems in robt tele operations. hey is it interesting to think about meta-decision makers,}
% Our research takes this human - AI joint decision making studies a step further by integrating confidence into the decision-making process of the dynamic robotic task. We created a simulation environment where humans interact with robots with varying delay factor in completing spatiotemporal rescue tasks, and a confidence-calibrated AI agent was there to assist human in robot decision-making. The task in focus involves selecting the optimal rescue robot for a specific control scenario where the robots have different delay characteristics. This delay injection concept reflects the reality that control signal transmission is aleatorically affected by the environment in which the robot is operating. In real-time robotic operations, decision-making process is critical, as delays can significantly affect performance, safety, and task completion. Even small delays in control can lead to substantial deviations from desired outcomes, such as imprecise movements, reduced efficiency, or even accidents. Ensuring that the right robot is chosen is vital for maintaining the reliability and effectiveness of robotic systems.  Our setup enables an in-depth exploration of human-AI decision-making dynamics in spatiotemporal robotic tasks and examines how shared confidence levels influence team decisions. Through this experiment, we evaluated human collaboration with AI agents in making critical decisions and assessed meta-decision-making methods, such as Maximum Confidence Slating (MCS), to improve team output.
% Agentic AI is focused on decisions as opposed to creating the actual new content, and doesn't solely rely on human input nor require human oversight \cite{shavit2023practices}. The drive for human-AI agent decision-making arises from the complementary strengths and abilities of humans and these computing machines. As we rapidly advance towards an AI-centric future, these AI agent systems are increasingly being utilized in collaboration with humans across a wide spectrum of decision-making domains, including healthcare, business, and design. One notable example of human-AI strategic decision-making is the PAL/CSS Freestyle Chess Tournament, where a lower-ranked player, supported by a medium-performance intelligence decision support system (IDS), outperformed a higher-ranked opponent with a marginally better ELO rating  \cite{chess2005}. Chess is, however, a fully observable, symmetric information game, in contrast to high-stakes decision-making tasks involving significant uncertainty and real-time operations, such as robotics. Similarly, most of the decision aids are currently deployed in static and passive tasks, for example, recidivism risk prediction~\cite{dss_whentoadvice,chiang2023two}, content moderation~\cite{keswani2021towards}, medical diagnosis~\cite{multiplehumans_ijcai22}, and rental price bidding~\cite{wang2023effects}, little is known about their integration into dynamic, complex and high-stake domain like robotics. These operational settings often involve prolonged cognitive strain \cite{zang2024large}, particularly in scenarios requiring teleoperated robotics for critical applications such as search-and-rescue missions, medical surgeries, military operations, hazardous material handling, and space exploration. In this high-stake scenarios, decision-making processes are pivotal for achieving optimal control, navigation, strategic goal and consistent task execution and can have profound impacts on human lives. 
% As semi- or fully autonomous teleoperated robots become increasingly integrated into industries - such as manufacturing (e.g., humanoid robots), healthcare (e.g., surgical robots), transportation (e.g., delivery robots), space exploration, and military applications (e.g., Palantir Gotham) \cite{palantir} - the need for precise and reliable real-time decision-making in selecting capable robots for long-term critical missions is crucial 
% \cite{cite dog military ICML}. 
Poor decisions can lead to inefficiencies, safety risks, or even failures in overall robotic operations. Given these high stakes, understanding how humans and AI can best collaborate in selecting capable mission-critical robots is essential and remain challenging, particularly in ensuring that these joint decision-making systems work effectively to improve outcomes in real-time robotic operations.
% In addition, optimizing this partnership to improve decision accuracy and efficiency in scenarios involving robot control with varying competence levels, so that it can be effectively implemented in real-world tasks, remains an open problem.
% Early robotic systems involving teleoperation relied solely on human operators as the decision-makers. Human decision-making, however, often relies on intuition, which can be susceptible to biases, emotions, and incomplete information \cite{casper2003human,norton2017analysis}. This can result in the gradual degradation of decision-making performance, particularly in complex, fast-paced, and long-term teleoperation scenarios. AI, while powerful, often lacks the contextual understanding and intuition that humans have. Recent advancements have sought to address these limitations by integrating AI decision support systems with the aim of enhancing decision accuracy through human-AI collaborative decision-making processes, particularly in scenarios involving high cognitive demands~\cite{hawes2017strands,kunze2018artificial,rigter2020framework}. At the outset, human-AI joint decision-making has been managed by a setup with human-initiative control~\cite{chiou2021mixed,hawes2007towards}, where the final decision to accept or reject the AI recommendation lies with the human operator.  Few have delved into the domain of joint decision-making, where both human and AI have an active role, especially in the context of real-time robotics control.

In our research, we explore the human joint decision-making
% \footnote{The meta decision-making refers to the higher-level decision about the decision-making process itself. It's essentially human making choices about when to use AI assistance in the overall human decision-making process. Example: human makes meta decision after observing AI suggestions.} 
% and meta joint decision-making \footnote{The meta joint decision-making refers to the decision whether to use AI decision or human decision in the overall decision-making process.} 
in the mix-initiative human-AI systems \cite{chiou2021mixed} in robot teleoperation tasks via integrating confidence-calibration\footnote{Confidence-accuracy calibration, or confidence-calibration is referred to as the metacognitive sensitivity in human psychology domain by Fleming et al.,\cite{fleming2014measure}
sharing into the decision-making process. This has been quantified by Area Under Curve-Receiver Operating Characteristics type 2 (AUROC2) measurement~\cite{nguyen2025confidence}}. We constructed a simulation environment where humans navigates multiple robots with varying delay factor in completing spatiotemporal tasks, and the AI-DSS was there to assist human in deciding the optimal robot for completing the navigation task. 
% \an{The choice for delay injection concept reflects the reality that control signal transmission is aleatorically affected by the environment in which the robot is operating. In real-time robotic operations, delays is critical and can significantly affect performance, safety, and task completion. Even small delays in control can lead to substantial deviations from desired outcomes, such as imprecise movements, reduced efficiency, and guaranteed accidents. Ensuring that the high performance robot is chosen is vital for maintaining the reliability and effectiveness of robotic systems. Our setup enables an in-depth exploration of human-AI decision-making dynamics in spatiotemporal robotic tasks and examines how shared metacognition sensitivity sharing influence team decision-making accuracy. }
Through this experiment, we evaluated human collaboration with various types of AI in joint decision-making and assessed the performance of algorithmic joint decision-making methods, such as Maximum Confidence Slating (MCS), in enhancing joint decision-making accuracy. Additionally, we measured the impact of confidence alignment\footnote{Confidence alignment refers to the degree of coherence between the confidence levels of humans and AI in the decision-making process. The coherence measurement is measure via distributional distance.} between humans and AI on the accuracy of joint decision-making.

% We investigate joint decision-making capabilities through three critical dimensions: Alignment, Task Di, and AI Confidence-Calibration.
% either human operators or fully autonomous AI systems. However, there's growing interest in joint decision-making between humans and AI, particularly in scenarios where neither humans nor AI alone can achieve the best decision-maker in long term mission [clarisaa paper]. This approach leverages the unique capabilities of both human intuition and AI's data processing power to navigate complex long term robotic environments and tasks more effectively.
% \an{include confidence alignment introduction and MCS}

% \an{reduce delay part}

Our study yields the following significant findings:

\begin{enumerate}[label=(\roman*)]

    \item Joint decisions decided by human, particularly when misalignment arise between humans and AI, underperform compared to MCS algorithm ($p < 0.001$). 
    % , utilizing an accessible metric like confidence ratings, offers an effective alternative for meta-decision maker in joint decision-making. 
    This marks the first application of the MCS in the context of human-AI joint decision-making within robotics.

    \item The varying AI confidence-calibration quality significantly affects team's joint decision-making accuracy ($p<0.01$). 
    % efficacy of confidence-sharing methods like MCS varies significantly with decision-making task difficulty and the AI confidence-calibration quality affects joint decision outcomes.
        
    \item Misalignment between human and AI confidence \\significantly impairs joint decision-making accuracy ($p < 0.001$). 




\end{enumerate}

% \begin{enumerate}
%     \item \textbf{Human Suboptimality}: One of our key findings is that human meta-decision\footnote{A meta-decision refers to a higher-level decision about the decision-making process itself. It's essentially making choices about when to use AI assistance in the overall decision-making process.}, when disagreement arises between humans and AI, is not the highest performing and can be outperformed by an algorithm. There is potential for a more effective approach through Maximum Confidence Slating (MCS) via an easy access metric: confidence. This is significant because it marks the first application of this algorithm in the context of human-AI joint decision-making within robotics for resolving disagreements.
%     \item \textbf{Perception Does Not Significantly Alter Behavior}: Interestingly, whether humans believe their teammate is an AI or another human does not statistically change their willingness to take advice in this robotics domain. This insight challenges assumptions about the impact of AI perception on decision-making. \cite{zhang2022you}
%     \item \textbf{Positive Impact of Even Suboptimal AI}: Pairing humans with AI, even when the AI is not perfectly confidence-calibrated, can improve overall decision accuracy. This suggests that AI’s role in decision-making is not just about providing the right answer but also about enhancing the decision-making process itself through confidence sharing.
%     \item \textbf{Importance of AI Confidence Calibration}: Finally, our research underscores the importance of well-calibrated AI confidence levels. A high-quality AI agent that accurately represents its confidence can lead to better decision outcomes, emphasizing that AI needs to be not only precise but also transparent about its certainty.
% \end{enumerate}
